Coupling Perovskite Quantum Dot Pairs in Solution using Nanoplasmonic Assembly

Perovskite quantum dots (PQDs) provide a robust solution-based approach to efficient solar cells, bright light-emitting devices, and quantum sources of light. Quantifying heterogeneity and understanding coupling between dots is critical for these applications. We use double-nanohole optical trapping to size individual dots and correlate to emission energy shifts from quantum confinement. We were able to assemble a second dot in the trap, which allows us to observe the coupling between dots. We observe a systematic red-shift of 1.1 $\pm$ 0.6 meV in the emission wavelength. Theoretical analysis shows that the observed shift is consistent with resonant energy transfer and is unusually large due to moderate-to-large quantum confinement in PQDs. This demonstrates the promise of PQDs for entanglement in quantum information applications. This work enables future in situ control of PQD growth as well as studies of the coupling between small PQD assemblies with quantum information applications in mind.

==> latexmkrc <==
add_cus_dep( 'tex', 'aux', 0, 'makeexternaldocument' );

sub makeexternaldocument {
    # if the dependency isn't one of the files that this latexmk run will consider, process it
    # without this test, we would get an infinite loop!
    if (!($root_filename eq $_[0]))
    {   # PLEASE ENABLE ONLY ONE OF THE FOLLOWING
        # DEPENDING ON THE ENGINE YOU'RE USING
    
        # FOR PDFLATEX
        system( "latexmk -pdf \"$_[0]\"" );

        # FOR LATEX+DVIPDF
        # system( "latexmk \"$_[0]\"" );

        # FOR XELATEX
        # system( "latexmk -xelatex \"$_[0]\"" );
        
        # FOR LUALATEX
        # system( "latexmk -lualatex \"$_[0]\"" );
   }
}
